Gridless Parameter Estimation in Partly Calibrated Rectangular Arrays

Spatial frequency estimation from a mixture of noisy sinusoids finds applications in various fields. While subspace-based methods offer cost-effective super-resolution parameter estimation, they demand precise array calibration, posing challenges for large antennas. In contrast, sparsity-based approaches outperform subspace methods, especially in scenarios with limited snapshots or correlated sources. This study focuses on direction-of-arrival (DOA) estimation using a partly calibrated rectangular array with fully calibrated subarrays. A gridless sparse formulation leveraging shift invariances in the array is developed, yielding two competitive algorithms under the alternating direction method of multipliers (ADMM) and successive convex approximation frameworks, respectively. Numerical simulations show the superior error performance of our proposed method, particularly in highly correlated scenarios, compared to the conventional subspace-based methods. It is demonstrated that the proposed formulation can also be adopted in the fully calibrated case to improve the robustness of the subspace-based methods to the source correlation. Furthermore, we provide a generalization of the proposed method to a more challenging case where a part of the sensors is unobservable due to failures.

==> images/arrayParams.tex <==
% set styles
\tikzset{
  antenna/.style = {circle,draw=TUDa-1b,fill=TUDa-1a,inner sep=1.5pt},
  axis/.style = {thick, -latex}
}
\def\xtick#1#2#3{
  \draw[thick,color=TUDa-8a] ($ #1 + (0,0.2) $) -- ($ #1 - (0,0.2) $) node[below,black] {}; % {$ \zeta_{#2,#3} $};
}
\def\ytick#1#2#3{
  \draw[thick,color=TUDa-8a] ($ #1 + (0.2,0) $) -- ($ #1 - (0.2,0) $) node[left,black] {}; % {$ \xi_{#2,#3} $};
}

% \def\subarrayXlist{0,4,9};	% relative subarray positions in x-axis
% \def\subarrayYlist{0,2};	% relative subarray positions in y-axis

\tikzmath{
	% array geometric parameters
	% \nSubarrayX = 3;	% number of subarrays along x-axis
	% \nSubarrayY = 2;	% number of subarrays along y-axis
  \nSubarray = 3;  % number of subarrays
  \subarrayXcoord1 = 0; \subarrayXcoord2 = 5; \subarrayXcoord3 = 9; % x-coordinates of subarrays
  \subarrayYcoord1 = 0; \subarrayYcoord2 = 1; \subarrayYcoord3 = 0; % y-coordinates of subarrays
	\nSensorX = 3;		% number of sensors along x-axis in each subarray
	\nSensorY = 2; 		% number of sensors along y-axis in each subarray
	\spaceX = 1;		% relative sensor spacing along x-axis within subarray
	\spaceY = 0.7;		% relative sensor spacing along y-axis within subarray	
	\x0 = 2;			% starting point for placing antennas in x-axis
	\y0 = 1.7;			% starting point for placing antennas in y-axis
  % compuate the maximum x and y coordinates of the sensors
  int \jx,\jy,\iSubarray;
  \xmax = \x0; \ymax = \y0; % maximum x and y coordinates
  for \iSubarray in {1,...,\nSubarray}{
    \subarrayX = \subarrayXcoord\iSubarray; % x coordinate of subarray \isubarray
    \subarrayY = \subarrayYcoord\iSubarray; % y coordinate of subarray \isubarray
    for \jx in {1,...,\nSensorX}{	% numeric calculation is not allowed in {list} here
      for \jy in {1,...,\nSensorY}{
        \sensorX = \x0+\subarrayX+\jx*\spaceX-\spaceX; % x coordinate of sensor
        \sensorY = \y0+\subarrayY+\jy*\spaceY-\spaceY; % y coordinate of sensor
        \xmax = max(\xmax, \sensorX); % update maximum x coordinate
        \ymax = max(\ymax, \sensorY); % update maximum y coordinate
      };
    };
  };
}


==> images/sensors.tex <==
% Use tikzmath for computations. Statements inside tikzmath must end with a semicolon.
% Keep comments ASCII-only to avoid input-encoding pitfalls inside tikzmath.
\tikzmath{
  int \jx,\jy,\iSubarray;
  % \xmax = \x0; \ymax = \y0; % maximum x and y coordinates
  %%%%%%%%%% draw antennas
  for \iSubarray in {1,...,\nSubarray}{
    \subarrayX = \subarrayXcoord\iSubarray; % x coordinate of subarray \isubarray
    \subarrayY = \subarrayYcoord\iSubarray; % y coordinate of subarray \isubarray
    for \jx in {1,...,\nSensorX}{	% numeric calculation is not allowed in {list} here
      for \jy in {1,...,\nSensorY}{
        \sensorX = \x0+\subarrayX+\jx*\spaceX-\spaceX; % x coordinate of sensor
        \sensorY = \y0+\subarrayY+\jy*\spaceY-\spaceY; % y coordinate of sensor
        % \xmax = max(\xmax, \sensorX); % update maximum x coordinate
        % \ymax = max(\ymax, \sensorY); % update maximum y coordinate
        { % draw antenna
          \node[antenna] at (\sensorX,\sensorY) {};	% () is not allowed in the coordinates here
        };
      };
    };
  };
  % \xlast = \x0+\subarrayX+\jx*\spaceX-\spaceX;	% x coordinate of last antenna
  % \ylast = \y0+\subarrayY+\jy*\spaceY-\spaceY;	% y coordinate of last antenna
}

